SynthRef: Generation of Synthetic Referring Expressions for Object Segmentation

Recent advances in deep learning have brought significant progress in visual grounding tasks such as language-guided video object segmentation. However, collecting large datasets for these tasks is expensive in terms of annotation time, which represents a bottleneck. To this end, we propose a novel method, namely SynthRef, for generating synthetic referring expressions for target objects in an image (or video frame), and we also present and disseminate the first large-scale dataset with synthetic referring expressions for video object segmentation. Our experiments demonstrate that by training with our synthetic referring expressions one can improve the ability of a model to generalize across different datasets, without any additional annotation cost. Moreover, our formulation allows its application to any object detection or segmentation dataset.

==> sections/2_Related_Work.tex <==
\section{Related Work}
\label{sec:relatedwork}

\noindent
\textbf{Referring Image Segmentation}
\quad
The task of segmenting objects or regions in images, given a referring expression, was introduced by \citet{hu2016segmentation}, who use a Convolutional Neural Network (CNN) and a Long Short-Term Memory (LSTM) network for extracting a visual and a language embedding respectively and combine them in order to obtain the segmentation mask of the referred object. To better exploit the correlations between words and image regions, \citet{liu2017recurrent} combine visual and word features with an LSTM to recurrently refine the segmentation masks. Dynamic filters were used by \citet{margffoy2018dynamic} and \citet{chen2019referring} to capture the recursive nature of language and the spatial information of the target object respectively. \citet{li2018referring} presented a recurrent refinement network (RRN) which refines the segmentation result by utilizing the feature pyramid structures in order to take advantage of multi-scale semantics. Posterior works in referring image segmentation leverage attention to model the visual information of each word. MAttNet~\citep{yu2018mattnet} decomposes referring expressions using three modules related to the object's appearance, location and relationships with other objects and then uses both language and visual attention to direct each module to focus on the desired part of the expression and the image. \citet{shi2018key} use attention to extract keywords from a referring expression which are important for identifying the target object. Cross-modal self-attention is used in CMSA~\citep{ye2019cross} to better capture the long-range dependencies between linguistic and visual features. While STEP~\citep{chen2019see} works in the same direction, it also uses a convRNN~\citep{xingjian2015convolutional} to refine the textual representation and improve the segmentation. A recent work by \citet{hu2020bi} proposes a bi-directional cross-modal attention module to learn the relationship between multi-modal features. Finally, \citet{huang2020referring} use multi-modal graph reasoning to identify the correct object as well as suppress other irrelevant ones.

\noindent
\textbf{Referring Video Object Segmentation}
\quad
Despite the increasing interest in referring image segmentation, a few works have explored the segmentation of objects using referring expressions in the video domain \ie Referring Video Object Segmentation. \citet{khoreva2018video} were the first to transfer the referring expression segmentation task from images to videos by collecting referring expressions for the DAVIS-2017~\citep{Pont-Tuset_arXiv_2017} dataset. They use the image-based MAttNet~\citep{yu2018mattnet} model pretrained on RefCOCO~\citep{kazemzadeh2014referitgame} to localize the target object, and then train a segmentation network with DAVIS-2017 to produce the pixel-wise prediction, using also temporal coherency across frames. \citet{gavrilyuk2018actor}, in a relevant work, provide natural language sentences for A2D~\citep{XuHsXiCVPR2015} and J-HMDB~\citep{Jhuang:ICCV:2013} which are datasets used for action and human pose recognition and segmentation. They employ a 3D fully-convolutional model with dynamic filters in order to segment an actor in each frame of a video as specified by a language query. Although the task is similar to referring video object segmentation, the referring expressions they provide are intended for describing an actor and its action. The first large scale-benchmark for referring video object segmentation, called Refer-YouTube-VOS, has been concurrently created by \citet{seourvos} on top of YouTube-VOS~\citep{xu2018youtube}, a benchmark for video object segmentation. Besides the dataset, the authors propose a model called URVOS, which performs language-based object segmentation  and  mask  propagation  jointly  using  a  single  deep  neural  network. The network combines a cross-modal attention module, inspired by CMSA~\citep{ye2019cross} and a memory attention module to encourage temporal consistency across frames.
In another concurrent work, RefVOS~\citep{bellver2020refvos} has been the first to leverage BERT~\citep{devlin2019bert}, a bidirectional transformer model for language understanding, for encoding the referring expressions. They have shown that using BERT instead of a bidirectional LSTM fed with GloVe embeddings~\citep{pennington2014glove}, which is a common practice in related works, brings significant improvements to the final segmentation. We use RefVOS in order to show the advantages of training a model with our synthetic referring expressions.



\noindent
\textbf{Synthetic Data}
\quad
Synthesizing training data has been explored in numerous applications in the fields of computer vision and natural language processing. The need of large amounts of data to train CNNs has encouraged the generation of synthetic datasets for solving tasks where real data cannot be easily collected. Flying Chairs~\citep{dosovitskiy2015flownet} and SURREAL~\citep{varol2017learning} are examples of synthetic datasets effectively used together with real data for the tasks of optical flow and human pose and shape estimation, respectively. \citet{peng2015learning} augmented existing datasets for few-shot object detection by synthesizing images from freely available 3D CAD models of objects. While on the aforementioned works synthetic and real data are mixed, \citet{saleh2018effective} proposed an effective way to use only synthetic data for semantic segmentation, by differentiating between foreground and background classes and using a detection-based approach. An enhanced Generative Adversarial Network (GAN) was used by \citet{shrivastava2017learning} aiming to reduce the domain gap between real and synthetic images. The authors showed the effectiveness of their method in the tasks of gaze and hand pose estimation. In a more recent work, \citet{khoreva2019lucid} recommend a training strategy using fewer in-domain than large-scale out-of-domain data, by exploiting the provided annotation on the first frame of a video to synthesize realistic future video frames.

Synthetic language data have also been used for training deep models on vision \& language tasks. \citet{fried2018speaker} proposed a speaker-follower model to synthesize instructions for the task of vision-and-language-navigation. \citet{silberer2018grounding} addressed the task of visual semantic role labeling and proved the effectiveness of training with synthetic data automatically created by applying a natural language processing model to image captions. The closest works to ours is PhraseCut~\citep{Wu_2020_CVPR} whose authors take advantage of the object categories, attributes and relationships annotated in the Visual Genome~\citep{krishna2017visual} dataset in order to create referring expressions which they use for the task of language-guided image segmentation. The difference of our work is that we automatically generate linguistic referring expressions using only the object categories and bounding boxes as ground truth annotations, and thus our idea can be used in any existing dataset that includes labeled object categories and bounding boxes.


